Predicting the trajectory of intracranial pressure in patients with traumatic brain injury: evaluation of a foundation model for time series

Patients with traumatic brain injury (TBI) often experience pathological increases in intracranial pressure (ICP), leading to intracranial hypertension (tIH), a common and serious complication. Early warning of an impending rise in ICP could potentially improve patient outcomes by enabling preemptive clinical intervention. However, the limited availability of patient data poses a challenge in developing reliable prediction models. In this study, we aim to determine whether foundation models, which leverage transfer learning, may offer a promising solution.

==> old.tex <==
\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 8.86 & 1.73 & 3.95 & 9.57 \\
LSTM & 8.75 & 1.65 & 3.84 & 9.49 \\
SES & 21.88 & 2.94 & 6.41 & 14.95 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on training set run 1}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 8.43 & 1.73 & 3.85 & 8.85 \\
LSTM & 8.78 & 1.84 & 3.82 & 9.00 \\
SES & 21.69 & 2.99 & 6.38 & 14.70 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on training set run 2}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 7.59 & 1.58 & 3.61 & 8.89 \\
LSTM & 8.05 & 1.56 & 3.58 & 9.49 \\
SES & 20.20 & 2.79 & 6.11 & 14.95 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on training set run 3}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 6.73 & 1.49 & 3.42 & 8.44 \\
LSTM & 6.82 & 1.48 & 3.34 & 8.58 \\
SES & 18.13 & 2.68 & 5.76 & 14.17 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on training set run 4}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 7.23 & 1.57 & 3.49 & 8.64 \\
LSTM & 7.21 & 1.53 & 3.40 & 8.62 \\
SES & 19.20 & 2.76 & 5.88 & 14.64 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on training set run 5}
\end{table} 




\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 6.34 & 1.50 & 3.29 & 8.34 \\
LSTM & 6.01 & 1.39 & 3.06 & 8.30 \\
SES & 16.00 & 2.53 & 5.42 & 14.06 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on validation set run 1}
\end{table}

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 6.02 & 1.35 & 3.04 & 8.93 \\
LSTM & 10.26 & 1.86 & 3.39 & 16.28 \\
SES & 16.64 & 2.45 & 5.32 & 14.53 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on validation set run 2}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 7.80 & 1.79 & 3.69 & 7.69 \\
LSTM & 8.30 & 1.81 & 3.84 & 7.85 \\
SES & 19.04 & 3.06 & 5.88 & 12.30 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on validation set run 3}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 14.76 & 2.37 & 4.80 & 12.63 \\
LSTM & 15.33 & 2.34 & 4.72 & 12.86 \\
SES & 35.92 & 3.98 & 8.38 & 16.68 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on validation set run 4}
\end{table} 

\begin{table}[]
\centering
\label{tab:training_performance}
\begin{tabular}{|l|l|l|l|l|}
\hline
Model & MSE & MAE & 90 percentile MAE & 99 percentile MAE  \\
\hline
Moment & 10.63 & 1.91 & 4.52 & 9.95 \\
LSTM & 11.14 & 1.85 & 4.53 & 10.55 \\
SES & 25.19 & 3.18 & 7.13 & 14.85 \\
\hline
\end{tabular}
\caption{Comparison of ML Model Performance Metrics on validation set run 5}
\end{table} 
